Tight Auditing of Differentially Private Machine Learning

Auditing mechanisms for differential privacy use probabilistic means to empirically estimate the privacy level of an algorithm. For private machine learning, existing auditing mechanisms are tight: the empirical privacy estimate (nearly) matches the algorithm's provable privacy guarantee. But these auditing techniques suffer from two limitations. First, they only give tight estimates under implausible worst-case assumptions (e.g., a fully adversarial dataset). Second, they require thousands or millions of training runs to produce non-trivial statistical estimates of the privacy leakage. This work addresses both issues. We design an improved auditing scheme that yields tight privacy estimates for natural (not adversarially crafted) datasets -- if the adversary can see all model updates during training. Prior auditing works rely on the same assumption, which is permitted under the standard differential privacy threat model. This threat model is also applicable, e.g., in federated learning settings. Moreover, our auditing scheme requires only two training runs (instead of thousands) to produce tight privacy estimates, by adapting recent advances in tight composition theorems for differential privacy. We demonstrate the utility of our improved auditing schemes by surfacing implementation bugs in private machine learning code that eluded prior auditing techniques.

==> DP auditing/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> DP auditing/new_methods.tex <==
\section{Auditing with \fdp}

\borja{Would be nice to include a (meta-)algorithm in this section explaining how the different algorithms in the rest of the paper are combined to produce lower bounds.}
To audit the privacy of DP-SGD, an adversary repeatedly runs a distinguishing attack to infer if a model's training set was either $D$ or $D'$; by measuring the false positive and false negative rates of the attack we can bound privacy.
All prior work has used $(\varepsilon, \delta)$-DP definition to audit the privacy parameters of the algorithm. 
The limitation of this approach is that different differential privacy mechanisms with \emph{identical} $(\varepsilon, \delta)$ guarantees can have \emph{different} trade-offs between false positive and false negative rates, which are upper bounded by the trade-off function of $(\varepsilon, \delta)$-differential privacy.
In particular, any $(\epsilon, \delta)$-DP guarantee corresponds to two symmetric supporting linear functions defining the trade-off between type I and type II errors.
However, any mechanism will have its own ``true'' trade-off curve capturing the relationship between the FPR and TPR of the best possible attack on the mechanism, consisting of the intersection between a collection of $(\epsilon, \delta(\epsilon))$-DP curves where $(\epsilon, \delta(\epsilon))$ satisfy \Cref{eps_gdp_convert}.
% \todo{Nicholas: you haven't defined adp at all. I don't know why you're saying we don't use somthing that's not defined.\milad{are you refereing to the \adp defintion ? we had it in section 2.1, but I rewrite it to make it a bit more obvious}}
While it is possible to audit any algorithm to lower bound its privacy with an \adp guarantee, we instead use an \fdp guarantee that is as close as possible to the true trade-off function of the mechanism.
By doing so, we can avoid any looseness that appears in converting between this \fdp guarantee and its collection of many \adp guarantees.
%A $\mu$-GDP mechanism's trade-off curve is instead given by the intersection of the collection of $(\epsilon, \delta(\epsilon))$-DP curves where $(\epsilon, \delta(\epsilon))$ satisfy \Cref{eps_gdp_convert}.
%By auditing with $\mu$-GDP we can exploit the fact that this formulation of differential privacy will give tighter control over the trade-off between type I and type II errors with a single parameter $\mu$ rather than attempting to lower bound the collection of $(\epsilon, \delta(\epsilon))$-DP guarantees simultaneously.
%\borja{My perspective on this is a bit different: most mechanisms satisfy a collection of guarantees $(\epsilon(\delta), \delta)$-DP or $(\epsilon, \delta(\epsilon))$-DP for varying values of $\delta$ or $\epsilon$, and previous auditing methods fail to exploit that. For example, if you take the "polygonal" regions coming from fixed parameter DP and intersect them all for all the valid values $(\epsilon, \delta(\epsilon))$-DP you will recover the more precise mechanism-specific curves from \Cref{fig:diff_mechanism_tradeoff}. Using, eg, GDP gives you a tighter curve controlled by a single parameter, which is why it's advantegeous for auditing instead of trying to lower bound all the $(\epsilon, \delta(\epsilon))$-DP curves at once.}
%\jhnote{Added something}
%\mcj{one way to frame this could be to talk about the ``true'' tradeoff function of a mechanism, and then later mention that the true tradeoff function for our attacks is much closer to gdp than it is to eps delta}

To illustrate this idea, in \Cref{fig:diff_mechanism_tradeoff} we plot the trade-off functions for several different DP mechanisms that all satisfy \adp where $\varepsilon=1,\delta=10^{-5}$. 
Clearly, the achievable false positive and false negative rates by an adversary who wants to audit a \adp guarantee depends significantly on the underlying privacy mechanism. 

\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figures/fig_mechansim_tradeoff.pdf}
    \caption{Comparison of the trade-of functions for different DP mechanisms that satisfy \adp where $\varepsilon=1,\delta=10^{-5}$. Note that the trade-off curve for the Random-Response mechanism overlaps with \adp.}
    \label{fig:diff_mechanism_tradeoff}
    \vspace{-0.7cm}
\end{figure}

Let us now give a concrete example demonstrating the benefit of auditing by measuring the privacy region of the private mechanism directly, rather than focusing on the privacy region specified by \adp. 
Suppose we want to audit an instance of the Gaussian mechanism satisfying $(1,10^{-5})$-DP; Figure~\ref{fig:dp_vs_fdp} illustrates the privacy regions of a generic private mechanism with $\varepsilon=1,\delta=10^{-5}$ and with a Gaussian mechanism which has an equivalent \adp guarantee (i.e, $\mu$-GDP with $\mu\approx0.25$). 
% As we can see in the figure, the privacy  region of a Gaussian mechanism is different from an unspecified mechanism that satisfies the same \adp privacy guarantee.
Now, if we want to audit the Gaussian mechanism by bounding \adp, our attack needs to have very low false positive or false negative rates (corresponding to the four locations where the GDP region and the \adp region have tangent borders). 
As a concrete example, suppose we are auditing this Gaussian mechanism (with $\varepsilon=1$) and we have an attack that achieves FPR$\approx0.23$ and FNR$=1- $FPR$ (e^{0.3}+\delta)$ over an infinite number of trials (the red dot in Figure~\ref{fig:dp_vs_fdp}).
If we use \adp to audit this mechanism we get an empirical $\epsilon$ of $0.3$, and we might (incorrectly) conclude that our mechanism is not tight. 
This is not because our attack is weak, but rather it is because our attack has a large FNR and no attack can achieve a lower FNR from the definition of the Gaussian mechanism (i.e, if an attack can achieve a lower FNR it violates $\sim0.25$-GDP). 

% If one can design an attack that reaches the optimal FPR, then can use either \adp or $\mu$-GDP to audit the mechanism, this might not be possible in practice. 
% First, to have an attack we a very small FPR, we need many trials to be able to get to even calculate the small FPR. 
% Second, working with high precision have potential risk of numerical instability and error which make it difficult to work with. 
% Moreover, most of the existing works use membership inference attacks~\cite{} which are optimized for average case accuracy~\cite{}.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.35]{figures/gdp_vs_dp_eps=1.pdf}
    \caption{Comparison of the privacy region of \adp vs \fdp for the Gaussian mechanism (GDP) with the same $\varepsilon$ budget.}
    \label{fig:dp_vs_fdp}
\end{figure}


\subsection{Lower Bounding \fdp With Clopper-Pearson}\label{ssec:lb_with_cp}
% \todo{Nicholas: It's not obvious to me that you're still doing f-DP but with clopper pearson. I'd start by making that obvious.}
Previous works use \Cref{eq: nasr_lb} which describe the predictive power of an adversary auditing with \adp to compute the privacy parameters from the false positive and negative rates. 
However, as we have already seen by appealing to the hypothesis testing interpretation of DP, the predictive power of the adversary is by definition equal to the trade-off function of the privacy mechanism. 
Therefore, instead of using \Cref{eq: nasr_lb} to compute the privacy parameters, we can directly use the trade-off function. 
Now by upper bounding the false positive ($\alpha$) and false negative rates ($\beta$) (referred to as $\bar{\alpha},\bar{\beta}$) we can calculate the lower bound on the privacy of the mechanism. 
Similar to the previous works~\cite{nasr2021adversary} we can use the Clopper-Pearson method to compute the upper bounds on the attacker errors.
 
For example, suppose we want to audit the Gaussian mechanism.  To compute a lower bound on the privacy parameters of the Gaussian mechanism (i.e, $\mu$), we have:
%

\begin{align}
    \mu_{emp}^{lower}   = \Phi^{-1}(1-\bar{\alpha})-\Phi^{-1}(\bar{\beta}) \;
\end{align}


%

We convert this into a lower bound for $\epsilon$ by noticing that the lower bound $\mu_{emp}^{lower}$ implies an upper bound on the trade-off function of the mechanism at every $\alpha$. 
Such an upper bound on the trade-off function enables us to use \Cref{eq:eps_delta_tradeoff} at a fixed $\delta$, to find the largest lower bound for $\epsilon$ over all $\alpha$.
 

\begin{figure*}
\centering
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps1.pdf}
    \caption{$\varepsilon=1$}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps2.pdf}
    \caption{$\varepsilon=2$}
    \end{subfigure}
    \begin{subfigure}{0.25\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps4.pdf}
    \caption{$\varepsilon=4$}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps6.pdf}
    \caption{$\varepsilon=6$}
    \end{subfigure}
\caption{Comparison of the \adp definition to audit DP-SGD compared to using \fdp of Gaussian mechanism both converted in \adp and lower bounded using Clopper Pearson (20 independent runs, $\delta=10^{-5}$).}
\label{fig:audit_gdp_dp}
\end{figure*}


\paragraph{Improvement:}
    Nasr et al.~\cite{nasr2021adversary} showed DP-SGD accounting is tight for a worst case dataset ($D=\emptyset$), assuming the adversary has white-box access to all iterations of the training. 
    However, they require many observations to achieve tight bounds, due to the aforementioned drawbacks of auditing with \adp.
    We re-evaluate this setting using our new approach of auditing with GDP. 
    In \Cref{fig:audit_gdp_dp}, we compare the lower bounds found through \adp (\Cref{eq: nasr_lb}) against using the Gaussian trade-off function and converting the Gaussian mechanism parameter to \adp, and we inspect how these two methods compare as the adversary collects more observations from which they compute upper bounds $\bar{\alpha}$ and $\bar{\beta}$.
    While, it is possible for \adp audit to find a lower bound that is tight to the theoretical value for $\epsilon$, this is only achieved when the adversary has 100 million observations. 
    When the number of the observations is smaller there is a non-trivial gap between the theoretical bound and the empirical lower bound.
    Comparatively, if we use the Gaussian mechanism's trade-off function (GDP) to estimate a lower bound on the privacy parameter $\mu$, and convert this into a bound on $\epsilon$, we can achieve a tight estimate even with 1,000 observations. 
    % Moreover, by using the trade-off function of the privacy mechanism instead of the generic \adp the auditing is less sensitive to the decision threshold that the auditor uses to compute the false/true positive rates.
    % Figure~\ref{fig: threshold_comparison_nsamples_5000} shows result of the auditing for different choices of threshold either using GDP or \adp. 
    % As we can see auditing using \adp is much more sensitive to the decision threshold compared to GDP.  
    % We discuss this in more detail in \Cref{app:choose_threshold}.
    %In our experiment section, we show how by using this technique we can achieve tight results in more detail other settings as well.

% \begin{figure}[t]
% %  \captionsetup{width=1.\textwidth, justification=centering}
% \centering
%     \includegraphics[width=1.\linewidth]{figures/compare_gdp_and_cp.pdf}
% \caption{We compare \fdp and \adp with Clopper-Pearson lower bounds for $5K$ observations. The lower bound found through GDP are approximately the same for any decision threshold within the observation's support, whereas the \adp with Clopper-Pearson lower bound varies dramatically. We also visualize observations when the canary was and wasn't included in training as histograms.}
% % we used $\delta=10^{-5}$}\tas{$\delta=10^{-5}$?}
% \label{fig: threshold_comparison_nsamples_5000}
% \end{figure}





\paragraph{Approximating the trade off function:}  While using GDP to audit can give us a tight lower bound on the estimated privacy in worst case settings, analyzing the privacy cost of a complex mechanism such as DP-SGD (that needs both sub-sampling amplification and composition over multiple update steps) is non-trivial. Dong et al.~\cite{dong2019gaussian} suggest to use a Central Limit Theorem for DP to compute a closed form solution, unfortunately, this can lead to significant underestimation of the privacy cost in general settings~\cite{koskela2020computing}. 
Therefore, to analyze DP-SGD we use an empirical approach called the ``Privacy Loss Distribution (PLD)''\cite{koskela2020computing} to approximate the trade-off function, which
computes a tight\milad{exact ?} privacy cost of DP-SGD over multiple update steps. 
We refer to Koskela et al.~\cite{koskela2020computing} for a detailed description of PLD, and will interact with it as a black-box $\varepsilon=f_{\mathcal{M}}(\delta)$ that for private mechanism $\mathcal{M}$ and a given $\delta$ will return the exact theoretical $\epsilon$. PLD does not have a closed-form trade-off function, in Appendix~\ref{app:pld} we explain how we use PLD for auditing.
 




\subsection{Lower Bounding \fdp With Bayesian Estimation}\label{ssec:baysian}

Recently, Zanella-Béguelin et al.~\cite{zanella2022bayesian} showed it is also possible to compute \emph{credible intervals} for $\epsilon$ using a Bayesian method which can significantly reduce the number of observations to estimate a tight bound. 
Here, we show it is possible to extend their approach to lower bound in \fdp (and then convert to a lower bound for $\epsilon$).

\begin{definition} [Cumulative Distribution Function of $f(\alpha,\hat{.})$-DP] Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR). The value of cumulative distribution function of $f(\alpha;\hat{.})$ evaluated at $f(\alpha;.)$ is:
%
\begin{equation}\label{eq:fdp_privacy}
    P_{\hat{.}}(.) = \int_{f(\alpha;.)}^{1-f(1-\alpha;.)} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \mathop{\wrt\alpha} \mathop{\wrt\beta}
\end{equation}

\end{definition}

Using \cref{eq:fdp_privacy}, we can find an empirical lower bound for $\mu$ in $\mu$-GDP, and then convert to a lower bound for \adp. 
As shown by Zanella-Béguelin et al.~\cite{zanella2022bayesian}, using the CDF of the private mechanism parameters given the attack observations of we can compute credible intervals over $\epsilon$. 
As a reminder Zanella-Béguelin et al.~defined  $u_{(\text{FPR,FNR})} $ as follows:
%
\begin{align}
    u_{(\text{FPR,FNR})}(\alpha,\beta) := & u_{(\text{FPR|FP})}(\alpha) u_{(\text{FNR|FN})}(\beta)  &\\
    = &\text{Beta}(\alpha;0.5 + \fn,0.5 +\n - \fn) \times& \nonumber  \\
    &\text{Beta}(\beta;0.5 + \fp,0.5 +\n - \fp) &\nonumber
\end{align}

where $\n\xspace$ is the number of observations used to compute false positive and false negative rates, and $\fn$, $\fp\xspace$ are the total number of false negative and false positives, respectively.

\milad{@borja can you add some explanation why this not valid}
    
% \paragraph{Gaussian Differential Privacy: }
% Given that Gaussian mechanism is one of the most common private mechanism, we instantiate the CDF of Gaussian mechanism as follow:

% \begin{definition}[Cumulative Distribution Function of $\mu'$-GDP]  Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR)~\cite{}. The value of cumulative distribution function of $\mu'$-GDP evaluated at $\mu$-GDP is :

% \begin{equation}\label{eq:gdp_privacy}
%     P_{\mu'}(\mu) = \int_{\Phi(\Phi^{-1}(1-\alpha)-\mu)}^{\Phi(\mu-\Phi^{-1}(\alpha))} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \wrt\alpha\ \wrt\beta
% \end{equation}

% \end{definition}


==> DP auditing/old_method.tex <==
\section{Lower Bounding DP-SGD} \label{sec:lower}

\subsection{Functional Differential Privacy}
Empirically evaluating differential privacy heavily depends on calculating tight confidence bounds on the estimated privacy bounds. 
Earlier works~\cite{} computed confidence intervals by computing lower and upper intervals on the false positive rates. Recently, Zanella-Béguelin et. al~\cite{} showed it is also possible to compute \emph{credible intervals} using a Bayesian method which can reduce the number of examples to estimate a tight bound significantly. 
In this work, we improve on their mechanism by measuring the privacy region of the private mechanism directly, rather than focusing on the privacy region of $(\varepsilon,\delta)$-differential privacy. 
To show why this is very important  w.l.o.g let's assume we want to audit a Gaussian mechanism with $(1,10^{-5})$-dp, Figure~\ref{fig:dp_vs_fdp} illustrates the privacy regions of a generic private mechanism with $\varepsilon=1,\delta=10^{-5}$ and with a Gaussian mechanism which has equivalent $(\varepsilon,\delta)$ (i.e, $\mu$-GDP with $\mu\approx0.25$). As we can see in the figure, the privacy  region of a Gaussian mechanism is different from an unspecified mechanism that satisfies the same $(\varepsilon,\delta)-$DP privacy guarantee.

Now, if we want to audit the Gaussian mechanism using $(\varepsilon,\delta)$-DP, we need to design an attack such that it can have very low false positive or false negative rates (there is only four optimal points where GDP and DP regions borders are tangent). To make this clear, let's consider that we are auditing this Gaussian mechanism (with $\varepsilon=1$) and we have attack that gets FPR$\approx0.23$ and FNR$=1- $FPR$ (e^{0.3}+\delta)$ over infinite number of trials (the red dot in Figure~\ref{fig:dp_vs_fdp}). If we use  $(\varepsilon,\delta)$-DP definition to audit this mechanism we get empirical epsilon of $0.3$. Which we might wrongly conclude that our mechanism is not tight. Please note this is not because our attack is weak is it is  because our attack has a large false negative rate and no attack can achieve lower FNR from the definition Gaussian mechanism (i.e, if an attack can achieve lower FNR it volates $\sim0.25$-GDP). While if we can have an attack which get the optimal FPR, we can use either $(\varepsilon,\delta)$-DP or $\mu$-GDP or audit the mechanism, this might not be possible in practice. First, to have an attack we a very small FPR, we need many trials to be able to get to even calculate the small FPR. Second, working with high precision have potential risk of numerical instability and error which make it difficult to work with. Moreover, most of the existing works use membership inference attacks~\cite{} which are optimized for average case accuracy~\cite{}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/gdp_vs_dp_eps=1.pdf}
    \caption{Comparison of the privacy region of $(\varepsilon,\delta)$-DP vs Functional Differential Privacy for Gaussian mechanism (GDP) for same $\varepsilon$ budget}
    \label{fig:dp_vs_fdp}
\end{figure}


Now that we argue that we should use functional differential privacy to audit different private mechanisms (e.g, using GDP to audit Gaussian mechanisms), we need to calculate the credible intervals for a given mechanism. We reformulate the work of  Zanella-Béguelin et. al~\cite{} for functional differential privacy which derives credible intervals for parameters of the f-DP from a given (FNR,FPR).




\begin{definition} [Cumulative Distribution Function of $f(\alpha,\hat{.})$-DP] Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR)~\cite{}. The value of cumulative distribution function of $f(\alpha;\hat{.})$ evaluated at $f(\alpha;.)$ is :

\begin{equation}\label{eq:fdp_privacy}
    P_{\hat{.}}(.) = \int_{f(\alpha;.)}^{1-f(1-\alpha;.)} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \wrt\alpha\ \wrt\beta
\end{equation}

\end{definition}

As explained in the previous work~\cite{}, using the CDF of private mechanism parameters given the attack observations of (FPR,FNR) we can compute the credible intervals which can be used as the confidence intervals. As a reminder Zanella-Béguelin et. al~\cite{} showed we define  $u_{(\text{FPR,FNR})} $ as follow:
\begin{align}
    u_{(\text{FPR,FNR})}(\alpha,\beta) := & u_{(\text{FPR|FP})}(\alpha) u_{(\text{FNR|FN})}(\beta)  &\\
    = &\text{Beta}(\alpha;0.5 + \fn,0.5 +\n - \fn) \times& \nonumber  \\
    &\text{Beta}(\beta;0.5 + \fp,0.5 +\n - \fp) &\nonumber
\end{align}
    
\subsection{Gaussian Differential Privacy}
Given that Gaussian mechanism is one of the most common private mechanism, we instantiate the CDF of Gaussian mechanism as follow:

\begin{definition}[Cumulative Distribution Function of $\mu'$-GDP]  Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR)~\cite{}. The value of cumulative distribution function of $\mu'$-GDP evaluated at $\mu$-GDP is :

\begin{equation}\label{eq:gdp_privacy}
    P_{\mu'}(\mu) = \int_{\Phi(\Phi^{-1}(1-\alpha)-\mu)}^{\Phi(\mu-\Phi^{-1}(\alpha))} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \wrt\alpha\ \wrt\beta
\end{equation}

\end{definition}

To show case the effectiveness of this approach, let's start with a simple one dimension function with sensitivity of $1$ and we use Gaussian mechanism mechanism with $\sigma=1$. Now the problem is to audit this simple mechanism when we have 1,000 trials where the half of trials is on dataset $D$ where the input to Gaussian mechanism is $0$ and other half on $D'$ with the input of $1$. Now using hypothesis testing with different threshold, we can get FPR-FNR curve as shown in Figure~\ref{fig:fnr_fpr_gdp_var1}. The we can use the observed FN and FP to calculate a lower bound on the epsilon. Figure~\ref{fig::dp_gdp_lower} compares the empirical lower bound of epsilon when we use $(\varepsilon,\delta)$-DP~\cite{} compared to $\mu$-GDP (Equation~\ref{eq:gdp_privacy}) and converted to $(\varepsilon,\delta)$-DP (using Corollary~\ref{eq:gdp_dp}). As shown in the figure when we use $(\varepsilon,\delta)$-DP definition to calculate the confidence bounds, the best estimates comes from having a high precision or recall attack, however, when the attack have lower precision/recall it get much smaller. Please note that in many attack scenarios (e.g. membership inference attack on machine learning~\cite{}) attack does not have high precision/recall and as result using them for auditing Gaussian mechanism will results in much loser lower bound when we use $(\varepsilon,\delta)$-DP privacy region. but it can improved significantly by using GDP.

\begin{figure*}
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[scale=0.44]{figures/gaussian-var1.pdf}
    \caption{The FPR-FNR curve for the }
    \label{fig:fnr_fpr_gdp_var1}
\end{minipage}
\hfill
\begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.41]{figures/gdp_vs_dp_lower_bound.pdf}
    \caption{lower bound estimation}
    \label{fig::dp_gdp_lower}
\end{minipage}
\end{figure*}

While using Gaussian differential privacy can gives us a tight lower bound on the estimated privacy, however, using GDP to analyze the privacy cost of the complex mechanism such as DP-SGD (that needs both subsampling amplification and composition) is non-trivial. Dong et al.~\cite{} suggested to use Central Limit Theorem to compute a closed formed solution, unfortunately, this can lead to significant under estimation of the privacy cost in general settings~\cite{}. Therefore, to analyze DP-SGD we use other definitions of differential privacy.

\subsection{Approximating Trade off Function }
Instead of using GDP, we can use Privacy Loss Distribution (PLD)~\cite{} to analyze the privacy cost of the DP-SGD. PLD compute the a tight (\milad{exact ?} ) privacy cost of the DP-SGD using numerical approaches. 
 PLD approaches does not have a closed-form trade-off function, but we can evaluate empirically lower bound them for each given FPR. However, since we need numerically compute Equation~\ref{eq:fdp_privacy}, it would be computationally expensive. Instead, we approximate the trade-off function using Algorithm~\ref{alg:pld_approx}. This will give us loser bound on the epsilon, but the difference is in the order of $10^{-1}$. 

\begin{algorithm}
\caption{Approximating a lower bound on trade-off function using PLD}\label{alg:pld_approx}
\begin{algorithmic}
\State \textbf{Args:} $f_{\mathcal{M}}$ privacy analysis function (outputs $\epsilon$ for a given $\delta$) , $n$ number of approximation lines, $\delta$ target delta in privacy analysis
\State $\Delta \gets n$ linearly spaced points between $[ \delta , 1-\delta ] $
\For {$\delta' \in \Delta $ }
\State $\hat{\varepsilon} \gets f_{\mathcal{M}}(\delta')$
\State $l_{\delta'}(x):= \max(0, 1-\delta'-(x  e^{\hat{\varepsilon}}), e^{-\hat{\varepsilon}(1-\delta'-x) } ) $
\EndFor 
\State $l(x) := \min_{\delta' \in \Delta} l_{\delta'} (x)$ \\
\Return $l$
\end{algorithmic}
\end{algorithm}


\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/pld_approx.pdf}
    \caption{Comparison of the trade-off fucntions when using the an approximation of PLD compared to optimal curve.}
    \label{fig:pld_apprix_compare}
\end{figure}


Figure~\ref{fig:pld_apprix_compare} compares the approximation approach in Algorithm~\ref{alg:pld_approx} to optimal trade-off function, as we can see, even with 10 approximation we can get a good estimation of the trade-off function. 





% \section{Threat Model}


% Similar to the previous work, we evaluate different threat models and settings to audit the DP-SGD algorithms. Previous work require to train many models to achieve the reasonable lower bound of the theoretical epsilon. In Section~\ref{sec:lower} we introduced several ideas to reduce the number of required models. 


% Nasr et al~\cite{} followed the exact 





% \begin{protocol}
% \centering
% \begin{tabular}{lcrr}
% \multicolumn{3}{c}{\textbf{ Adversary Game}} \\
% \textbf{Adversary}\hspace{2em} & \hspace{3em} & \textbf{Model Trainer} \\
% \cmidrule{1-3}
%  & & $b \sample \{0, 1\}$ \\
% \multicolumn{3}{c}{\sendmessageleft{top={$f_{\theta_{0}}$}}} \\
% \multicolumn{2}{l}{$\mathcal{G}, \mathcal{G} \cup \{g'\} \sample \mathcal{A}(f_{\theta_i}) $ } & &
% \rdelim\}{4}{*}[\rotatebox{90}{\hspace{-3em}Repeat $N$ Iterations}] \\
% \multicolumn{3}{c}{\sendmessageright{top={$ \mathcal{B}^{i} \gets \{ \mathbb{B}(\mathcal{G}) , \mathbb{B}(\mathcal{G}) \cup {G}\} $},bottom={$\Pr[G=\{g'\}]=q_i,\Pr[G=\emptyset]=1-q_i $ }}} \\
% & & $B \gets \mathcal{B}_{b^i }^i$ \\
% &\multicolumn{2}{r}{$B_{dp} \gets \{\text{clip}_p(x) + N \,\colon\,x \in B\}$} &\\
% &\multicolumn{2}{r}{$\theta_{i+1} \gets \theta_{i} - \eta \sum_{x \in B_{dp}} x$}&  \\
% \multicolumn{3}{c}{\sendmessageleft{top={$f_{\theta_{i+1}}$}}} \\
% & \vdots & \\


% \multicolumn{2}{l}{$s \gets \mathcal{B}(\{f_{\theta_i}\}, \mathcal{G})$} & & \\
% \multicolumn{3}{c}{\sendmessageright{top={$s \in \{0,1\}$}}} \\
% & & Check if $s=b$ \\
% \end{tabular}
% \caption{\textbf{Overall Adversary game for auditing attack.} }
%     \label{fig:overall_protocol}
% \end{protocol}
 
 
 

% Protocol~\ref{fig:overall_protocol} summarizes the overall view of our auditing setup. There are several differences between our setup 


% \subsection{Adversary's Capability}
%  While this setting might not be practical, we can use this for auditing ... By using this setting, we can have a tight estimation of epsilon which helps to prevent such errors without the need to train several models. Since we are only auditing one single iteration of the DP-SGD training a full model will give us many observations and we only need to train a 



\subsection{Auditing Individual Steps of DP-SGD }
DP-SGD is an iterative algorithm, previous works  focused on auditing this algorithm by using the information after the model has been trained (a single observation comes from one training run). 
In this work, we argue in cases where we have access to the intermediate steps, it is beneficial to audit each iteration of the DP-SGD algorithm individually. 
Doing so allows us to use different iterations of the DP-SGD algorithm to estimate a lower bound on the privacy cost of each iteration. 
In other words, we do not need to train multiple models to have an estimate for the DP-SGD mechanism and we only need to pay about twice the computation cost (in most cases) to be able to get a tight lower bound. 
If we want to audit the total privacy spent over training, we can compute a lower bound for a single iteration and then compose this to compute the overall cost.


\begin{proposition}\label{prop:emprical_composition}
write mathy stuff about the lower bound on the one step is still correct on the overall budget because of PLD ...
\end{proposition}


% \subsection{How to find $\bar{\alpha}$ and $\bar{\beta}$ in practice}

% \jhnote{This is a mess but I think we need a description like this}
% The adversary collects $n$ instances of $\mathcal{M}(D)$, $X_{D} = \{\mathcal{M}(D)_1, \mathcal{M}(D)_2, \ldots, \mathcal{M}(D)_n\}$ and $n$ instances of $\mathcal{M}(D')$, $X_{D'} = \{\mathcal{M}(D')_1, \mathcal{M}(D')_2, \ldots, \mathcal{M}(D')_n\}$.
% Given $X_D$ and $X_{D'}$, the adversary designs a transformation function $T:\text{Range}(\mathcal{M})\rightarrow \mathcal{T}$, that transforms $\mathcal{M}(D)$ into a new space $\mathcal{T}$.
% For example, if TODO
% The adversary also defines a decision function $\phi:\mathcal{T}\rightarrow \{0, 1\}$, such that $\phi{T(\mathcal{M}(D))}=0$ and $\phi{T(\mathcal{M}(D'))}=1$.
% Most commonly \cite{}, $T$ is defined as the loss of the differing point under a model trained with $D$ or $D'$, and $\phi$ is a parameterized by threshold $\phi$ from which we assign TODO  

\begin{algorithm}
\caption{DP-SGD with {\color{ForestGreen} gradient} or {\color{Cerulean} input} space auditing in with white-box access }\label{alg:dpsgd_debug}
\begin{algorithmic}
\State \textbf{Args:}  training dataset $D$, sampling rate $q$, learning rate $\eta$, noise scale $\sigma$, gradient norm clip $C$, loss function $l$, {\color{ForestGreen} canary gradient $g'$}, {\color{Cerulean} canary input $(x', y')$}, canary sampling rate $q_c$, function that clips gradients to a max norm $C$ \texttt{clip}
	\State Initiate $\theta$ randomly
	\State Observations: $\mathcal{O} \gets \{\}$, $\mathcal{O}' \gets \{\}$
	\For{$t \in \{T\}$}
	\State $B_t \gets$ sample instances from dataset $D$ with prob $q$
	\State $B'_t \gets$ sample instances from dataset $D$ with prob $q$
	
	\State $\nabla [t] \gets \vec{0}$ 
	\ForAll{$ (x,y)  \in B_t$}
	\State $\nabla[t] \gets \nabla [t]+ \text{\texttt{clip}}(\nabla_{\theta}(l(x,y))) $
	
	\EndFor
	\State $\widetilde{\nabla[t]} \gets \nabla[t]  + \mathcal{N}(0,\sigma^2C^2\mathbb{I})   $
	
    \State $\nabla' [t] \gets \vec{0}$ 
	\ForAll{$ (x,y)  \in B'_t$}
	\State $\nabla'[t] \gets \nabla' [t]+ \text{\texttt{clip}}(\nabla_{\theta}(l(x,y))) $
	\EndFor
	
% 	\begingroup
%     \color{ForestGreen}
%     \State $g' \gets \text{canary gradient}$
%     \endgroup
	
	\begingroup
    \color{Cerulean}
    \State $g' \gets \text{\texttt{clip}}(\nabla_{\theta}(l(x',y')))$ 
    \endgroup
    
	\State $\nabla' [t] \gets \nabla' [t] + g' $ with prob $q_c$ o.w. $\nabla' [t] + \vec{0}$
	\State $\widetilde{\nabla'[t]} \gets \nabla'[t]  + \mathcal{N}(0,\sigma^2C^2\mathbb{I})   $
	
	\begingroup
    % \color{ForestGreen}
	\State $\mathcal{O}[t] \gets \langle  g', {\nabla[t]}\rangle$
	\State $\mathcal{O}'[t] \gets \langle  g', {\nabla'[t]}\rangle$
	\endgroup
	\State $\theta \gets \theta  - \eta \widetilde{\nabla[t]}$ 
% 	\begingroup
%     \color{Cerulean}
%     \State $\theta' \gets \theta  - \eta \widetilde{\nabla'[t]}$ 
% 	\State $\mathcal{O}[t] \gets l_{\theta}(x',y')$
% 	\State $\mathcal{O}'[t] \gets l_{\theta'}(x',y')$
% 	\endgroup
	
	\EndFor \\
	\Return $\theta$ , $\mathcal{O}$
\end{algorithmic}
\end{algorithm}

% \jhnote{This explanantion should come before the experimental section.}
% The model trainer goal is to use auditing to get an estimation of the privacy parameters. 
% Therefore, in this setting the adversary is the model trainer which has white-box access to the model in all steps of the training and can also modify the training parameters. 
% We design an strong adversary for this setting which reduces the computation complexity of the debugging. 
% First, instead of the estimating the overall privacy budget of the training, the adversary only audits an individual iteration. 
% Since the adversary is the the model trainer and it knows that the algorithm is repeating the same mechanism for each iteration and then it can only focus on one iteration as explained in Section~\ref{}.  
% Second, since the adversary can influence the training procedure. Therefore we modify the DP-SGD algorithm to~\cref{alg:dpsgd_debug} to include the debugging settings.

\milad{reread this to make sure it is understandable}
In each iteration of the DPSGD ~\cref{alg:dpsgd_debug}, the trainer selects two batches of data, $B$ and $B'$, and adds a canary sample to $B'$ with probability $q_c$. This means that $B$ is sampled from the original dataset $D$, while $B'$ is sampled from a modified dataset $D'$. The trainer then calculates the dot product between the noisy gradient and the canary for each batch, resulting in a score for each batch. The goal of the adversary is to determine whether a batch is from dataset $D$ or $D'$. At the end of each run of the algorithm, the trainer produces $T$ observations and a fully trained model with parameters $\theta$.




 ~\cref{alg:dpsgd_debug} uses different sampling rate for the canary example. This allow the model trainer to evaluate the mechanism at different sampling rates. Specially the model trainer can set $q_c$ to 1 which means the canary is selected in all iterations and the model trainer only focus on auditing the privacy mechanism without the sub-sampling. Auditing the batch sampling  of DP-SGD can be done using simpler auditing mechanism independent of DP-SGD. 


In the rare cases  that the model trainer is using different mechanism in different iterations then the adversary should only audit the iterations that use the same mechanism and compute the lower bound on different mechanisms separately. Since this is not commonly used in practice we do not explore this setting in our work.


==> new_methods.tex <==
\section{Auditing with \fdp}

\borja{Would be nice to include a (meta-)algorithm in this section explaining how the different algorithms in the rest of the paper are combined to produce lower bounds.}
To audit the privacy of DP-SGD, an adversary repeatedly runs a distinguishing attack to infer if a model's training set was either $D$ or $D'$; by measuring the false positive and false negative rates of the attack we can bound privacy.
All prior work has used $(\varepsilon, \delta)$-DP definition to audit the privacy parameters of the algorithm. 
The limitation of this approach is that different differential privacy mechanisms with \emph{identical} $(\varepsilon, \delta)$ guarantees can have \emph{different} trade-offs between false positive and false negative rates, which are upper bounded by the trade-off function of $(\varepsilon, \delta)$-differential privacy.
In particular, any $(\epsilon, \delta)$-DP guarantee corresponds to two symmetric supporting linear functions defining the trade-off between type I and type II errors.
However, any mechanism will have its own ``true'' trade-off curve capturing the relationship between the FPR and TPR of the best possible attack on the mechanism, consisting of the intersection between a collection of $(\epsilon, \delta(\epsilon))$-DP curves where $(\epsilon, \delta(\epsilon))$ satisfy \Cref{eps_gdp_convert}.
% \todo{Nicholas: you haven't defined adp at all. I don't know why you're saying we don't use somthing that's not defined.\milad{are you refereing to the \adp defintion ? we had it in section 2.1, but I rewrite it to make it a bit more obvious}}
While it is possible to audit any algorithm to lower bound its privacy with an \adp guarantee, we instead use an \fdp guarantee that is as close as possible to the true trade-off function of the mechanism.
By doing so, we can avoid any looseness that appears in converting between this \fdp guarantee and its collection of many \adp guarantees.
%A $\mu$-GDP mechanism's trade-off curve is instead given by the intersection of the collection of $(\epsilon, \delta(\epsilon))$-DP curves where $(\epsilon, \delta(\epsilon))$ satisfy \Cref{eps_gdp_convert}.
%By auditing with $\mu$-GDP we can exploit the fact that this formulation of differential privacy will give tighter control over the trade-off between type I and type II errors with a single parameter $\mu$ rather than attempting to lower bound the collection of $(\epsilon, \delta(\epsilon))$-DP guarantees simultaneously.
%\borja{My perspective on this is a bit different: most mechanisms satisfy a collection of guarantees $(\epsilon(\delta), \delta)$-DP or $(\epsilon, \delta(\epsilon))$-DP for varying values of $\delta$ or $\epsilon$, and previous auditing methods fail to exploit that. For example, if you take the "polygonal" regions coming from fixed parameter DP and intersect them all for all the valid values $(\epsilon, \delta(\epsilon))$-DP you will recover the more precise mechanism-specific curves from \Cref{fig:diff_mechanism_tradeoff}. Using, eg, GDP gives you a tighter curve controlled by a single parameter, which is why it's advantegeous for auditing instead of trying to lower bound all the $(\epsilon, \delta(\epsilon))$-DP curves at once.}
%\jhnote{Added something}
%\mcj{one way to frame this could be to talk about the ``true'' tradeoff function of a mechanism, and then later mention that the true tradeoff function for our attacks is much closer to gdp than it is to eps delta}

To illustrate this idea, in \Cref{fig:diff_mechanism_tradeoff} we plot the trade-off functions for several different DP mechanisms that all satisfy \adp where $\varepsilon=1,\delta=10^{-5}$. 
Clearly, the achievable false positive and false negative rates by an adversary who wants to audit a \adp guarantee depends significantly on the underlying privacy mechanism. 

\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figures/fig_mechansim_tradeoff.pdf}
    \caption{Comparison of the trade-of functions for different DP mechanisms that satisfy \adp where $\varepsilon=1,\delta=10^{-5}$. Note that the trade-off curve for the Random-Response mechanism overlaps with \adp.}
    \label{fig:diff_mechanism_tradeoff}
    \vspace{-0.7cm}
\end{figure}

Let us now give a concrete example demonstrating the benefit of auditing by measuring the privacy region of the private mechanism directly, rather than focusing on the privacy region specified by \adp. 
Suppose we want to audit an instance of the Gaussian mechanism satisfying $(1,10^{-5})$-DP; Figure~\ref{fig:dp_vs_fdp} illustrates the privacy regions of a generic private mechanism with $\varepsilon=1,\delta=10^{-5}$ and with a Gaussian mechanism which has an equivalent \adp guarantee (i.e, $\mu$-GDP with $\mu\approx0.25$). 
% As we can see in the figure, the privacy  region of a Gaussian mechanism is different from an unspecified mechanism that satisfies the same \adp privacy guarantee.
Now, if we want to audit the Gaussian mechanism by bounding \adp, our attack needs to have very low false positive or false negative rates (corresponding to the four locations where the GDP region and the \adp region have tangent borders). 
As a concrete example, suppose we are auditing this Gaussian mechanism (with $\varepsilon=1$) and we have an attack that achieves FPR$\approx0.23$ and FNR$=1- $FPR$ (e^{0.3}+\delta)$ over an infinite number of trials (the red dot in Figure~\ref{fig:dp_vs_fdp}).
If we use \adp to audit this mechanism we get an empirical $\epsilon$ of $0.3$, and we might (incorrectly) conclude that our mechanism is not tight. 
This is not because our attack is weak, but rather it is because our attack has a large FNR and no attack can achieve a lower FNR from the definition of the Gaussian mechanism (i.e, if an attack can achieve a lower FNR it violates $\sim0.25$-GDP). 

% If one can design an attack that reaches the optimal FPR, then can use either \adp or $\mu$-GDP to audit the mechanism, this might not be possible in practice. 
% First, to have an attack we a very small FPR, we need many trials to be able to get to even calculate the small FPR. 
% Second, working with high precision have potential risk of numerical instability and error which make it difficult to work with. 
% Moreover, most of the existing works use membership inference attacks~\cite{} which are optimized for average case accuracy~\cite{}.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.35]{figures/gdp_vs_dp_eps=1.pdf}
    \caption{Comparison of the privacy region of \adp vs \fdp for the Gaussian mechanism (GDP) with the same $\varepsilon$ budget.}
    \label{fig:dp_vs_fdp}
\end{figure}


\subsection{Lower Bounding \fdp With Clopper-Pearson}\label{ssec:lb_with_cp}
% \todo{Nicholas: It's not obvious to me that you're still doing f-DP but with clopper pearson. I'd start by making that obvious.}
Previous works use \Cref{eq: nasr_lb} which describe the predictive power of an adversary auditing with \adp to compute the privacy parameters from the false positive and negative rates. 
However, as we have already seen by appealing to the hypothesis testing interpretation of DP, the predictive power of the adversary is by definition equal to the trade-off function of the privacy mechanism. 
Therefore, instead of using \Cref{eq: nasr_lb} to compute the privacy parameters, we can directly use the trade-off function. 
Now by upper bounding the false positive ($\alpha$) and false negative rates ($\beta$) (referred to as $\bar{\alpha},\bar{\beta}$) we can calculate the lower bound on the privacy of the mechanism. 
Similar to the previous works~\cite{nasr2021adversary} we can use the Clopper-Pearson method to compute the upper bounds on the attacker errors.
 
For example, suppose we want to audit the Gaussian mechanism.  To compute a lower bound on the privacy parameters of the Gaussian mechanism (i.e, $\mu$), we have:
%

\begin{align}
    \mu_{emp}^{lower}   = \Phi^{-1}(1-\bar{\alpha})-\Phi^{-1}(\bar{\beta}) \;
\end{align}


%

We convert this into a lower bound for $\epsilon$ by noticing that the lower bound $\mu_{emp}^{lower}$ implies an upper bound on the trade-off function of the mechanism at every $\alpha$. 
Such an upper bound on the trade-off function enables us to use \Cref{eq:eps_delta_tradeoff} at a fixed $\delta$, to find the largest lower bound for $\epsilon$ over all $\alpha$.
 

\begin{figure*}
\centering
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps1.pdf}
    \caption{$\varepsilon=1$}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps2.pdf}
    \caption{$\varepsilon=2$}
    \end{subfigure}
    \begin{subfigure}{0.25\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps4.pdf}
    \caption{$\varepsilon=4$}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[scale=0.32]{figures/audit_gdp_dp_eps6.pdf}
    \caption{$\varepsilon=6$}
    \end{subfigure}
\caption{Comparison of the \adp definition to audit DP-SGD compared to using \fdp of Gaussian mechanism both converted in \adp and lower bounded using Clopper Pearson (20 independent runs, $\delta=10^{-5}$).}
\label{fig:audit_gdp_dp}
\end{figure*}


\paragraph{Improvement:}
    Nasr et al.~\cite{nasr2021adversary} showed DP-SGD accounting is tight for a worst case dataset ($D=\emptyset$), assuming the adversary has white-box access to all iterations of the training. 
    However, they require many observations to achieve tight bounds, due to the aforementioned drawbacks of auditing with \adp.
    We re-evaluate this setting using our new approach of auditing with GDP. 
    In \Cref{fig:audit_gdp_dp}, we compare the lower bounds found through \adp (\Cref{eq: nasr_lb}) against using the Gaussian trade-off function and converting the Gaussian mechanism parameter to \adp, and we inspect how these two methods compare as the adversary collects more observations from which they compute upper bounds $\bar{\alpha}$ and $\bar{\beta}$.
    While, it is possible for \adp audit to find a lower bound that is tight to the theoretical value for $\epsilon$, this is only achieved when the adversary has 100 million observations. 
    When the number of the observations is smaller there is a non-trivial gap between the theoretical bound and the empirical lower bound.
    Comparatively, if we use the Gaussian mechanism's trade-off function (GDP) to estimate a lower bound on the privacy parameter $\mu$, and convert this into a bound on $\epsilon$, we can achieve a tight estimate even with 1,000 observations. 
    % Moreover, by using the trade-off function of the privacy mechanism instead of the generic \adp the auditing is less sensitive to the decision threshold that the auditor uses to compute the false/true positive rates.
    % Figure~\ref{fig: threshold_comparison_nsamples_5000} shows result of the auditing for different choices of threshold either using GDP or \adp. 
    % As we can see auditing using \adp is much more sensitive to the decision threshold compared to GDP.  
    % We discuss this in more detail in \Cref{app:choose_threshold}.
    %In our experiment section, we show how by using this technique we can achieve tight results in more detail other settings as well.

% \begin{figure}[t]
% %  \captionsetup{width=1.\textwidth, justification=centering}
% \centering
%     \includegraphics[width=1.\linewidth]{figures/compare_gdp_and_cp.pdf}
% \caption{We compare \fdp and \adp with Clopper-Pearson lower bounds for $5K$ observations. The lower bound found through GDP are approximately the same for any decision threshold within the observation's support, whereas the \adp with Clopper-Pearson lower bound varies dramatically. We also visualize observations when the canary was and wasn't included in training as histograms.}
% % we used $\delta=10^{-5}$}\tas{$\delta=10^{-5}$?}
% \label{fig: threshold_comparison_nsamples_5000}
% \end{figure}





\paragraph{Approximating the trade off function:}  While using GDP to audit can give us a tight lower bound on the estimated privacy in worst case settings, analyzing the privacy cost of a complex mechanism such as DP-SGD (that needs both sub-sampling amplification and composition over multiple update steps) is non-trivial. Dong et al.~\cite{dong2019gaussian} suggest to use a Central Limit Theorem for DP to compute a closed form solution, unfortunately, this can lead to significant underestimation of the privacy cost in general settings~\cite{koskela2020computing}. 
Therefore, to analyze DP-SGD we use an empirical approach called the ``Privacy Loss Distribution (PLD)''\cite{koskela2020computing} to approximate the trade-off function, which
computes a tight\milad{exact ?} privacy cost of DP-SGD over multiple update steps. 
We refer to Koskela et al.~\cite{koskela2020computing} for a detailed description of PLD, and will interact with it as a black-box $\varepsilon=f_{\mathcal{M}}(\delta)$ that for private mechanism $\mathcal{M}$ and a given $\delta$ will return the exact theoretical $\epsilon$. PLD does not have a closed-form trade-off function, in Appendix~\ref{app:pld} we explain how we use PLD for auditing.
 




\subsection{Lower Bounding \fdp With Bayesian Estimation}\label{ssec:baysian}

Recently, Zanella-Béguelin et al.~\cite{zanella2022bayesian} showed it is also possible to compute \emph{credible intervals} for $\epsilon$ using a Bayesian method which can significantly reduce the number of observations to estimate a tight bound. 
Here, we show it is possible to extend their approach to lower bound in \fdp (and then convert to a lower bound for $\epsilon$).

\begin{definition} [Cumulative Distribution Function of $f(\alpha,\hat{.})$-DP] Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR). The value of cumulative distribution function of $f(\alpha;\hat{.})$ evaluated at $f(\alpha;.)$ is:
%
\begin{equation}\label{eq:fdp_privacy}
    P_{\hat{.}}(.) = \int_{f(\alpha;.)}^{1-f(1-\alpha;.)} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \mathop{\wrt\alpha} \mathop{\wrt\beta}
\end{equation}

\end{definition}

Using \cref{eq:fdp_privacy}, we can find an empirical lower bound for $\mu$ in $\mu$-GDP, and then convert to a lower bound for \adp. 
As shown by Zanella-Béguelin et al.~\cite{zanella2022bayesian}, using the CDF of the private mechanism parameters given the attack observations of we can compute credible intervals over $\epsilon$. 
As a reminder Zanella-Béguelin et al.~defined  $u_{(\text{FPR,FNR})} $ as follows:
%
\begin{align}
    u_{(\text{FPR,FNR})}(\alpha,\beta) := & u_{(\text{FPR|FP})}(\alpha) u_{(\text{FNR|FN})}(\beta)  &\\
    = &\text{Beta}(\alpha;0.5 + \fn,0.5 +\n - \fn) \times& \nonumber  \\
    &\text{Beta}(\beta;0.5 + \fp,0.5 +\n - \fp) &\nonumber
\end{align}

where $\n\xspace$ is the number of observations used to compute false positive and false negative rates, and $\fn$, $\fp\xspace$ are the total number of false negative and false positives, respectively.

\milad{@borja can you add some explanation why this not valid}
    
% \paragraph{Gaussian Differential Privacy: }
% Given that Gaussian mechanism is one of the most common private mechanism, we instantiate the CDF of Gaussian mechanism as follow:

% \begin{definition}[Cumulative Distribution Function of $\mu'$-GDP]  Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR)~\cite{}. The value of cumulative distribution function of $\mu'$-GDP evaluated at $\mu$-GDP is :

% \begin{equation}\label{eq:gdp_privacy}
%     P_{\mu'}(\mu) = \int_{\Phi(\Phi^{-1}(1-\alpha)-\mu)}^{\Phi(\mu-\Phi^{-1}(\alpha))} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \wrt\alpha\ \wrt\beta
% \end{equation}

% \end{definition}


==> old_method.tex <==
\section{Lower Bounding DP-SGD} \label{sec:lower}

\subsection{Functional Differential Privacy}
Empirically evaluating differential privacy heavily depends on calculating tight confidence bounds on the estimated privacy bounds. 
Earlier works~\cite{} computed confidence intervals by computing lower and upper intervals on the false positive rates. Recently, Zanella-Béguelin et. al~\cite{} showed it is also possible to compute \emph{credible intervals} using a Bayesian method which can reduce the number of examples to estimate a tight bound significantly. 
In this work, we improve on their mechanism by measuring the privacy region of the private mechanism directly, rather than focusing on the privacy region of $(\varepsilon,\delta)$-differential privacy. 
To show why this is very important  w.l.o.g let's assume we want to audit a Gaussian mechanism with $(1,10^{-5})$-dp, Figure~\ref{fig:dp_vs_fdp} illustrates the privacy regions of a generic private mechanism with $\varepsilon=1,\delta=10^{-5}$ and with a Gaussian mechanism which has equivalent $(\varepsilon,\delta)$ (i.e, $\mu$-GDP with $\mu\approx0.25$). As we can see in the figure, the privacy  region of a Gaussian mechanism is different from an unspecified mechanism that satisfies the same $(\varepsilon,\delta)-$DP privacy guarantee.

Now, if we want to audit the Gaussian mechanism using $(\varepsilon,\delta)$-DP, we need to design an attack such that it can have very low false positive or false negative rates (there is only four optimal points where GDP and DP regions borders are tangent). To make this clear, let's consider that we are auditing this Gaussian mechanism (with $\varepsilon=1$) and we have attack that gets FPR$\approx0.23$ and FNR$=1- $FPR$ (e^{0.3}+\delta)$ over infinite number of trials (the red dot in Figure~\ref{fig:dp_vs_fdp}). If we use  $(\varepsilon,\delta)$-DP definition to audit this mechanism we get empirical epsilon of $0.3$. Which we might wrongly conclude that our mechanism is not tight. Please note this is not because our attack is weak is it is  because our attack has a large false negative rate and no attack can achieve lower FNR from the definition Gaussian mechanism (i.e, if an attack can achieve lower FNR it volates $\sim0.25$-GDP). While if we can have an attack which get the optimal FPR, we can use either $(\varepsilon,\delta)$-DP or $\mu$-GDP or audit the mechanism, this might not be possible in practice. First, to have an attack we a very small FPR, we need many trials to be able to get to even calculate the small FPR. Second, working with high precision have potential risk of numerical instability and error which make it difficult to work with. Moreover, most of the existing works use membership inference attacks~\cite{} which are optimized for average case accuracy~\cite{}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/gdp_vs_dp_eps=1.pdf}
    \caption{Comparison of the privacy region of $(\varepsilon,\delta)$-DP vs Functional Differential Privacy for Gaussian mechanism (GDP) for same $\varepsilon$ budget}
    \label{fig:dp_vs_fdp}
\end{figure}


Now that we argue that we should use functional differential privacy to audit different private mechanisms (e.g, using GDP to audit Gaussian mechanisms), we need to calculate the credible intervals for a given mechanism. We reformulate the work of  Zanella-Béguelin et. al~\cite{} for functional differential privacy which derives credible intervals for parameters of the f-DP from a given (FNR,FPR).




\begin{definition} [Cumulative Distribution Function of $f(\alpha,\hat{.})$-DP] Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR)~\cite{}. The value of cumulative distribution function of $f(\alpha;\hat{.})$ evaluated at $f(\alpha;.)$ is :

\begin{equation}\label{eq:fdp_privacy}
    P_{\hat{.}}(.) = \int_{f(\alpha;.)}^{1-f(1-\alpha;.)} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \wrt\alpha\ \wrt\beta
\end{equation}

\end{definition}

As explained in the previous work~\cite{}, using the CDF of private mechanism parameters given the attack observations of (FPR,FNR) we can compute the credible intervals which can be used as the confidence intervals. As a reminder Zanella-Béguelin et. al~\cite{} showed we define  $u_{(\text{FPR,FNR})} $ as follow:
\begin{align}
    u_{(\text{FPR,FNR})}(\alpha,\beta) := & u_{(\text{FPR|FP})}(\alpha) u_{(\text{FNR|FN})}(\beta)  &\\
    = &\text{Beta}(\alpha;0.5 + \fn,0.5 +\n - \fn) \times& \nonumber  \\
    &\text{Beta}(\beta;0.5 + \fp,0.5 +\n - \fp) &\nonumber
\end{align}
    
\subsection{Gaussian Differential Privacy}
Given that Gaussian mechanism is one of the most common private mechanism, we instantiate the CDF of Gaussian mechanism as follow:

\begin{definition}[Cumulative Distribution Function of $\mu'$-GDP]  Let $u_{(\text{FPR,FNR})}$ be the density function of the joint distribution of (FPR,FNR)~\cite{}. The value of cumulative distribution function of $\mu'$-GDP evaluated at $\mu$-GDP is :

\begin{equation}\label{eq:gdp_privacy}
    P_{\mu'}(\mu) = \int_{\Phi(\Phi^{-1}(1-\alpha)-\mu)}^{\Phi(\mu-\Phi^{-1}(\alpha))} \int_{0}^1 u_{(\text{FPR,FNR})} (\alpha,\beta) \wrt\alpha\ \wrt\beta
\end{equation}

\end{definition}

To show case the effectiveness of this approach, let's start with a simple one dimension function with sensitivity of $1$ and we use Gaussian mechanism mechanism with $\sigma=1$. Now the problem is to audit this simple mechanism when we have 1,000 trials where the half of trials is on dataset $D$ where the input to Gaussian mechanism is $0$ and other half on $D'$ with the input of $1$. Now using hypothesis testing with different threshold, we can get FPR-FNR curve as shown in Figure~\ref{fig:fnr_fpr_gdp_var1}. The we can use the observed FN and FP to calculate a lower bound on the epsilon. Figure~\ref{fig::dp_gdp_lower} compares the empirical lower bound of epsilon when we use $(\varepsilon,\delta)$-DP~\cite{} compared to $\mu$-GDP (Equation~\ref{eq:gdp_privacy}) and converted to $(\varepsilon,\delta)$-DP (using Corollary~\ref{eq:gdp_dp}). As shown in the figure when we use $(\varepsilon,\delta)$-DP definition to calculate the confidence bounds, the best estimates comes from having a high precision or recall attack, however, when the attack have lower precision/recall it get much smaller. Please note that in many attack scenarios (e.g. membership inference attack on machine learning~\cite{}) attack does not have high precision/recall and as result using them for auditing Gaussian mechanism will results in much loser lower bound when we use $(\varepsilon,\delta)$-DP privacy region. but it can improved significantly by using GDP.

\begin{figure*}
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[scale=0.44]{figures/gaussian-var1.pdf}
    \caption{The FPR-FNR curve for the }
    \label{fig:fnr_fpr_gdp_var1}
\end{minipage}
\hfill
\begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.41]{figures/gdp_vs_dp_lower_bound.pdf}
    \caption{lower bound estimation}
    \label{fig::dp_gdp_lower}
\end{minipage}
\end{figure*}

While using Gaussian differential privacy can gives us a tight lower bound on the estimated privacy, however, using GDP to analyze the privacy cost of the complex mechanism such as DP-SGD (that needs both subsampling amplification and composition) is non-trivial. Dong et al.~\cite{} suggested to use Central Limit Theorem to compute a closed formed solution, unfortunately, this can lead to significant under estimation of the privacy cost in general settings~\cite{}. Therefore, to analyze DP-SGD we use other definitions of differential privacy.

\subsection{Approximating Trade off Function }
Instead of using GDP, we can use Privacy Loss Distribution (PLD)~\cite{} to analyze the privacy cost of the DP-SGD. PLD compute the a tight (\milad{exact ?} ) privacy cost of the DP-SGD using numerical approaches. 
 PLD approaches does not have a closed-form trade-off function, but we can evaluate empirically lower bound them for each given FPR. However, since we need numerically compute Equation~\ref{eq:fdp_privacy}, it would be computationally expensive. Instead, we approximate the trade-off function using Algorithm~\ref{alg:pld_approx}. This will give us loser bound on the epsilon, but the difference is in the order of $10^{-1}$. 

\begin{algorithm}
\caption{Approximating a lower bound on trade-off function using PLD}\label{alg:pld_approx}
\begin{algorithmic}
\State \textbf{Args:} $f_{\mathcal{M}}$ privacy analysis function (outputs $\epsilon$ for a given $\delta$) , $n$ number of approximation lines, $\delta$ target delta in privacy analysis
\State $\Delta \gets n$ linearly spaced points between $[ \delta , 1-\delta ] $
\For {$\delta' \in \Delta $ }
\State $\hat{\varepsilon} \gets f_{\mathcal{M}}(\delta')$
\State $l_{\delta'}(x):= \max(0, 1-\delta'-(x  e^{\hat{\varepsilon}}), e^{-\hat{\varepsilon}(1-\delta'-x) } ) $
\EndFor 
\State $l(x) := \min_{\delta' \in \Delta} l_{\delta'} (x)$ \\
\Return $l$
\end{algorithmic}
\end{algorithm}


\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/pld_approx.pdf}
    \caption{Comparison of the trade-off fucntions when using the an approximation of PLD compared to optimal curve.}
    \label{fig:pld_apprix_compare}
\end{figure}


Figure~\ref{fig:pld_apprix_compare} compares the approximation approach in Algorithm~\ref{alg:pld_approx} to optimal trade-off function, as we can see, even with 10 approximation we can get a good estimation of the trade-off function. 





% \section{Threat Model}


% Similar to the previous work, we evaluate different threat models and settings to audit the DP-SGD algorithms. Previous work require to train many models to achieve the reasonable lower bound of the theoretical epsilon. In Section~\ref{sec:lower} we introduced several ideas to reduce the number of required models. 


% Nasr et al~\cite{} followed the exact 





% \begin{protocol}
% \centering
% \begin{tabular}{lcrr}
% \multicolumn{3}{c}{\textbf{ Adversary Game}} \\
% \textbf{Adversary}\hspace{2em} & \hspace{3em} & \textbf{Model Trainer} \\
% \cmidrule{1-3}
%  & & $b \sample \{0, 1\}$ \\
% \multicolumn{3}{c}{\sendmessageleft{top={$f_{\theta_{0}}$}}} \\
% \multicolumn{2}{l}{$\mathcal{G}, \mathcal{G} \cup \{g'\} \sample \mathcal{A}(f_{\theta_i}) $ } & &
% \rdelim\}{4}{*}[\rotatebox{90}{\hspace{-3em}Repeat $N$ Iterations}] \\
% \multicolumn{3}{c}{\sendmessageright{top={$ \mathcal{B}^{i} \gets \{ \mathbb{B}(\mathcal{G}) , \mathbb{B}(\mathcal{G}) \cup {G}\} $},bottom={$\Pr[G=\{g'\}]=q_i,\Pr[G=\emptyset]=1-q_i $ }}} \\
% & & $B \gets \mathcal{B}_{b^i }^i$ \\
% &\multicolumn{2}{r}{$B_{dp} \gets \{\text{clip}_p(x) + N \,\colon\,x \in B\}$} &\\
% &\multicolumn{2}{r}{$\theta_{i+1} \gets \theta_{i} - \eta \sum_{x \in B_{dp}} x$}&  \\
% \multicolumn{3}{c}{\sendmessageleft{top={$f_{\theta_{i+1}}$}}} \\
% & \vdots & \\


% \multicolumn{2}{l}{$s \gets \mathcal{B}(\{f_{\theta_i}\}, \mathcal{G})$} & & \\
% \multicolumn{3}{c}{\sendmessageright{top={$s \in \{0,1\}$}}} \\
% & & Check if $s=b$ \\
% \end{tabular}
% \caption{\textbf{Overall Adversary game for auditing attack.} }
%     \label{fig:overall_protocol}
% \end{protocol}
 
 
 

% Protocol~\ref{fig:overall_protocol} summarizes the overall view of our auditing setup. There are several differences between our setup 


% \subsection{Adversary's Capability}
%  While this setting might not be practical, we can use this for auditing ... By using this setting, we can have a tight estimation of epsilon which helps to prevent such errors without the need to train several models. Since we are only auditing one single iteration of the DP-SGD training a full model will give us many observations and we only need to train a 



\subsection{Auditing Individual Steps of DP-SGD }
DP-SGD is an iterative algorithm, previous works  focused on auditing this algorithm by using the information after the model has been trained (a single observation comes from one training run). 
In this work, we argue in cases where we have access to the intermediate steps, it is beneficial to audit each iteration of the DP-SGD algorithm individually. 
Doing so allows us to use different iterations of the DP-SGD algorithm to estimate a lower bound on the privacy cost of each iteration. 
In other words, we do not need to train multiple models to have an estimate for the DP-SGD mechanism and we only need to pay about twice the computation cost (in most cases) to be able to get a tight lower bound. 
If we want to audit the total privacy spent over training, we can compute a lower bound for a single iteration and then compose this to compute the overall cost.


\begin{proposition}\label{prop:emprical_composition}
write mathy stuff about the lower bound on the one step is still correct on the overall budget because of PLD ...
\end{proposition}


% \subsection{How to find $\bar{\alpha}$ and $\bar{\beta}$ in practice}

% \jhnote{This is a mess but I think we need a description like this}
% The adversary collects $n$ instances of $\mathcal{M}(D)$, $X_{D} = \{\mathcal{M}(D)_1, \mathcal{M}(D)_2, \ldots, \mathcal{M}(D)_n\}$ and $n$ instances of $\mathcal{M}(D')$, $X_{D'} = \{\mathcal{M}(D')_1, \mathcal{M}(D')_2, \ldots, \mathcal{M}(D')_n\}$.
% Given $X_D$ and $X_{D'}$, the adversary designs a transformation function $T:\text{Range}(\mathcal{M})\rightarrow \mathcal{T}$, that transforms $\mathcal{M}(D)$ into a new space $\mathcal{T}$.
% For example, if TODO
% The adversary also defines a decision function $\phi:\mathcal{T}\rightarrow \{0, 1\}$, such that $\phi{T(\mathcal{M}(D))}=0$ and $\phi{T(\mathcal{M}(D'))}=1$.
% Most commonly \cite{}, $T$ is defined as the loss of the differing point under a model trained with $D$ or $D'$, and $\phi$ is a parameterized by threshold $\phi$ from which we assign TODO  

\begin{algorithm}
\caption{DP-SGD with {\color{ForestGreen} gradient} or {\color{Cerulean} input} space auditing in with white-box access }\label{alg:dpsgd_debug}
\begin{algorithmic}
\State \textbf{Args:}  training dataset $D$, sampling rate $q$, learning rate $\eta$, noise scale $\sigma$, gradient norm clip $C$, loss function $l$, {\color{ForestGreen} canary gradient $g'$}, {\color{Cerulean} canary input $(x', y')$}, canary sampling rate $q_c$, function that clips gradients to a max norm $C$ \texttt{clip}
	\State Initiate $\theta$ randomly
	\State Observations: $\mathcal{O} \gets \{\}$, $\mathcal{O}' \gets \{\}$
	\For{$t \in \{T\}$}
	\State $B_t \gets$ sample instances from dataset $D$ with prob $q$
	\State $B'_t \gets$ sample instances from dataset $D$ with prob $q$
	
	\State $\nabla [t] \gets \vec{0}$ 
	\ForAll{$ (x,y)  \in B_t$}
	\State $\nabla[t] \gets \nabla [t]+ \text{\texttt{clip}}(\nabla_{\theta}(l(x,y))) $
	
	\EndFor
	\State $\widetilde{\nabla[t]} \gets \nabla[t]  + \mathcal{N}(0,\sigma^2C^2\mathbb{I})   $
	
    \State $\nabla' [t] \gets \vec{0}$ 
	\ForAll{$ (x,y)  \in B'_t$}
	\State $\nabla'[t] \gets \nabla' [t]+ \text{\texttt{clip}}(\nabla_{\theta}(l(x,y))) $
	\EndFor
	
% 	\begingroup
%     \color{ForestGreen}
%     \State $g' \gets \text{canary gradient}$
%     \endgroup
	
	\begingroup
    \color{Cerulean}
    \State $g' \gets \text{\texttt{clip}}(\nabla_{\theta}(l(x',y')))$ 
    \endgroup
    
	\State $\nabla' [t] \gets \nabla' [t] + g' $ with prob $q_c$ o.w. $\nabla' [t] + \vec{0}$
	\State $\widetilde{\nabla'[t]} \gets \nabla'[t]  + \mathcal{N}(0,\sigma^2C^2\mathbb{I})   $
	
	\begingroup
    % \color{ForestGreen}
	\State $\mathcal{O}[t] \gets \langle  g', {\nabla[t]}\rangle$
	\State $\mathcal{O}'[t] \gets \langle  g', {\nabla'[t]}\rangle$
	\endgroup
	\State $\theta \gets \theta  - \eta \widetilde{\nabla[t]}$ 
% 	\begingroup
%     \color{Cerulean}
%     \State $\theta' \gets \theta  - \eta \widetilde{\nabla'[t]}$ 
% 	\State $\mathcal{O}[t] \gets l_{\theta}(x',y')$
% 	\State $\mathcal{O}'[t] \gets l_{\theta'}(x',y')$
% 	\endgroup
	
	\EndFor \\
	\Return $\theta$ , $\mathcal{O}$
\end{algorithmic}
\end{algorithm}

% \jhnote{This explanantion should come before the experimental section.}
% The model trainer goal is to use auditing to get an estimation of the privacy parameters. 
% Therefore, in this setting the adversary is the model trainer which has white-box access to the model in all steps of the training and can also modify the training parameters. 
% We design an strong adversary for this setting which reduces the computation complexity of the debugging. 
% First, instead of the estimating the overall privacy budget of the training, the adversary only audits an individual iteration. 
% Since the adversary is the the model trainer and it knows that the algorithm is repeating the same mechanism for each iteration and then it can only focus on one iteration as explained in Section~\ref{}.  
% Second, since the adversary can influence the training procedure. Therefore we modify the DP-SGD algorithm to~\cref{alg:dpsgd_debug} to include the debugging settings.

\milad{reread this to make sure it is understandable}
In each iteration of the DPSGD ~\cref{alg:dpsgd_debug}, the trainer selects two batches of data, $B$ and $B'$, and adds a canary sample to $B'$ with probability $q_c$. This means that $B$ is sampled from the original dataset $D$, while $B'$ is sampled from a modified dataset $D'$. The trainer then calculates the dot product between the noisy gradient and the canary for each batch, resulting in a score for each batch. The goal of the adversary is to determine whether a batch is from dataset $D$ or $D'$. At the end of each run of the algorithm, the trainer produces $T$ observations and a fully trained model with parameters $\theta$.




 ~\cref{alg:dpsgd_debug} uses different sampling rate for the canary example. This allow the model trainer to evaluate the mechanism at different sampling rates. Specially the model trainer can set $q_c$ to 1 which means the canary is selected in all iterations and the model trainer only focus on auditing the privacy mechanism without the sub-sampling. Auditing the batch sampling  of DP-SGD can be done using simpler auditing mechanism independent of DP-SGD. 


In the rare cases  that the model trainer is using different mechanism in different iterations then the adversary should only audit the iterations that use the same mechanism and compute the lower bound on different mechanisms separately. Since this is not commonly used in practice we do not explore this setting in our work.

